Oracle Complexity of Single-Loop Switching Subgradient Methods for Non-Smooth Weakly Convex Functional Constrained Optimization

We consider a non-convex constrained optimization problem, where the objective function is weakly convex and the constraint function is either convex or weakly convex. To solve this problem, we consider the classical switching subgradient method, which is an intuitive and easily implementable first-order method whose oracle complexity was only known for convex problems. This paper provides the first analysis on the oracle complexity of the switching subgradient method for finding a nearly stationary point of non-convex problems. Our results are derived separately for convex and weakly convex constraints. Compared to existing approaches, especially the double-loop methods, the switching gradient method can be applied to non-smooth problems and achieves the same complexity using only a single loop, which saves the effort on tuning the number of inner iterations.

==> macros.tex <==
% author defined macros, keep it simple and minimum
\newcommand{\X}{\mathcal{X}}
\newcommand{\bzt}{\boldsymbol{\zeta}}
\newcommand{\bog}{\boldsymbol{\omega}}
\newcommand{\Prob}{\text{Prob}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\minimize}{\mathop{\mathrm{minimize}{}}}
\newcommand{\maximize}{\mathop{\mathrm{maximize}{}}}
\newcommand{\argmin}{\mathop{\mathrm{arg\,min}{}}}
\newcommand{\argmax}{\mathop{\mathrm{arg\,max}{}}}
%\newcommand{\prox}{\mathrm{prox}}
\newcommand{\prox}{\mathbf{prox}}
\newcommand{\dom}{\mathrm{dom\,}}
%\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\eqdef}{\stackrel{\triangle}{=}}
\newcommand{\reals}{\mathbf{R}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\Expect}{\mathbf{E}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Bdiv}{\mathcal{B}}

% macros specific to this paper
\newcommand{\condbat}{\kappa_{\mathrm{bat}}}
\newcommand{\conddbat}{\kappa'_{\mathrm{bat}}}
\newcommand{\condrand}{\kappa_{\mathrm{rand}}}
\newcommand{\conddrand}{\kappa'_{\mathrm{rand}}}
\newcommand{\mtld}{\tilde{m}}
\newcommand{\Lagr}{{L}}
%\newcommand{\Lagr}{\mathcal{L}}
\newcommand{\pmin}{{p_\textrm{min}}}
\newcommand{\pmax}{{p_\textrm{max}}}
\newcommand{\qmin}{{q_\textrm{min}}}
\newcommand{\qmax}{{q_\textrm{max}}}
\newcommand{\Ptld}{\widetilde{P}}
\newcommand{\Dtld}{\widetilde{D}}
\newcommand{\aopt}{\alpha^{\star}}
\newcommand{\aini}{\alpha^{(0)}}
\newcommand{\at}{\alpha^{(t)}}
\newcommand{\aT}{\alpha^{(T)}}
\newcommand{\aM}{\alpha^{(M)}}
\newcommand{\atp}{\alpha^{(t+1)}}
\newcommand{\ai}{\alpha_i}
\newcommand{\aj}{\alpha_j}
\newcommand{\aiopt}{\alpha_i^{\star}}
\newcommand{\aiini}{\alpha_i^{(0)}}
\newcommand{\ait}{\alpha_i^{(t)}}
\newcommand{\aitp}{\alpha_i^{(t+1)}}
\newcommand{\ajt}{\alpha_j^{(t)}}
\newcommand{\anjt}{\alpha_{-j}^{(t)}}
\newcommand{\ajtp}{\alpha_j^{(t+1)}}
\newcommand{\aitld}{\tilde{\alpha}_{i}^{(t+1)}}
\newcommand{\aitldr}{\tilde{\alpha}_{i}^{(r)}}
\newcommand{\atld}{\tilde{\alpha}}
\newcommand{\atldopt}{\tilde{\alpha}^{\star}}
\newcommand{\atldini}{\tilde{\alpha}^{(0)}}
\newcommand{\atldr}{\tilde{\alpha}^{(r)}}
\newcommand{\atldrp}{\tilde{\alpha}^{(r+1)}}
\newcommand{\abs}{\bar{\alpha}^{(s)}}
\newcommand{\abS}{\bar{\alpha}^{(S)}}
\newcommand{\absp}{\bar{\alpha}^{(s+1)}}
\newcommand{\abiini}{\bar{\alpha}_{i}^{(0)}}
\newcommand{\abis}{\bar{\alpha}_{i}^{(s)}}
\newcommand{\abjs}{\bar{\alpha}_{j}^{(s)}}
\newcommand{\abini}{\bar{\alpha}^{(0)}}
\newcommand{\bit}{\beta_i^{(t)}}
\newcommand{\bitp}{\beta_i^{(t+1)}}
\newcommand{\biini}{\beta_i^{(0)}}
\newcommand{\jt}{{j^{(t)}}}
\newcommand{\jtp}{{j^{(t+1)}}}
\newcommand{\jtps}{{j^{(t+s)}}}
\newcommand{\lt}{{l^{(t)}}}
\newcommand{\ltp}{{l^{(t+1)}}}
\newcommand{\ltps}{{l^{(t+s)}}}
\newcommand{\uit}{{u_i^{(t)}}}
\newcommand{\uitp}{{u_i^{(t+1)}}}
\newcommand{\ujtp}{{u_j^{(t+1)}}}
\newcommand{\ubs}{\bar{u}^{(s)}}
\newcommand{\ubt}{\bar{u}^{(t)}}
\newcommand{\ubini}{\bar{u}^{(0)}}
\newcommand{\ubis}{\bar{u}_i^{(s)}}
\newcommand{\ubjs}{\bar{u}_j^{(s)}}
\newcommand{\ubit}{\bar{u}_i^{(t)}}
\newcommand{\ubitp}{\bar{u}_i^{(t+1)}}
\newcommand{\ubjt}{\bar{u}_j^{(t)}}
\newcommand{\ubjtp}{\bar{u}_j^{(t+1)}}
\newcommand{\vkt}{{v_k^{(t)}}}
\newcommand{\vktp}{{v_k^{(t+1)}}}
\newcommand{\vltp}{{v_l^{(t+1)}}}
\newcommand{\vbs}{\bar{v}^{(s)}}
\newcommand{\vbt}{\bar{v}^{(t)}}
\newcommand{\vbini}{\bar{v}^{(0)}}
\newcommand{\vbks}{\bar{v}_k^{(s)}}
\newcommand{\vbkt}{\bar{v}_k^{(t)}}
\newcommand{\vbktp}{\bar{v}_k^{(t+1)}}
\newcommand{\vbls}{\bar{v}_l^{(s)}}
\newcommand{\vblt}{\bar{v}_l^{(t)}}
\newcommand{\vbltp}{\bar{v}_l^{(t+1)}}
\newcommand{\wk}{{w_k}}
\newcommand{\wl}{{w_l}}
\newcommand{\wopt}{{w^{\star}}}
\newcommand{\wini}{{w^{(0)}}}
\newcommand{\wt}{{w^{(t)}}}
\newcommand{\wT}{{w^{(T)}}}
\newcommand{\wM}{{w^{(M)}}}
\newcommand{\wtp}{{w^{(t+1)}}}
\newcommand{\wkopt}{{w_k^{\star}}}
\newcommand{\wkini}{{w_k^{(0)}}}
\newcommand{\wkt}{{w_k^{(t)}}}
\newcommand{\wktp}{{w_k^{(t+1)}}}
\newcommand{\wlt}{{w_l^{(t)}}}
\newcommand{\wltp}{{w_l^{(t+1)}}}
\newcommand{\wktld}{\tilde{w}_{k}^{(t+1)}}
\newcommand{\wktldr}{\tilde{w}_{k}^{(r)}}
\newcommand{\wtld}{\tilde{w}}
\newcommand{\wtldopt}{\tilde{w}^{\star}}
\newcommand{\wtldini}{\tilde{w}^{(0)}}
\newcommand{\wtldr}{\tilde{w}^{(r)}}
\newcommand{\wtldrp}{\tilde{w}^{(r+1)}}
\newcommand{\wbs}{\bar{w}^{(s)}}
\newcommand{\wbS}{\bar{w}^{(S)}}
\newcommand{\wbsp}{\bar{w}^{(s+1)}}
\newcommand{\wbkini}{\bar{w}_k^{(0)}}
\newcommand{\wbks}{\bar{w}_k^{(s)}}
\newcommand{\wbls}{\bar{w}_l^{(s)}}
\newcommand{\wbini}{\bar{w}^{(0)}}
\newcommand{\ztld}{\tilde{z}}
\newcommand{\zopt}{{z}^{\star}}
\newcommand{\zini}{{z}^{(0)}}
\newcommand{\zit}{{z_i^{(t)}}}
\newcommand{\zt}{{z}^{(t)}}
\newcommand{\zbs}{\bar{z}^{(s)}}
\newcommand{\zbS}{\bar{z}^{(S)}}
\newcommand{\zbT}{\bar{z}^{(T)}}
\newcommand{\zbini}{\bar{z}^{(0)}}
\newcommand{\ztldini}{\tilde{z}^{(0)}}
\newcommand{\ztldr}{\tilde{z}^{(r)}}
\newcommand{\ztldrp}{\tilde{z}^{(r+1)}}
\newcommand{\ztldopt}{\tilde{z}^{\star}}
\newcommand{\ztldoptr}{\tilde{z}^{\star(r)}}
\newcommand{\Dt}{\Delta^{(t)}}
\newcommand{\DT}{\Delta^{(T)}}
\newcommand{\DM}{\Delta^{(M)}}
\newcommand{\Dtp}{\Delta^{(t+1)}}
\newcommand{\Dini}{\Delta^{(0)}}
\newcommand{\Dbini}{\bar{\Delta}^{(0)}}
\newcommand{\Dbs}{\bar{\Delta}^{(s)}}
\newcommand{\Dbsp}{\bar{\Delta}^{(s+1)}}
\newcommand{\Xik}{{X_{ik}}}
\newcommand{\Xil}{{X_{il}}}
\newcommand{\Xjl}{{X_{jl}}}
\newcommand{\Xjk}{{X_{jk}}}
\newcommand{\Xri}{{X_{i:}}}
\newcommand{\Xrj}{{X_{j:}}}
\newcommand{\Xck}{{X_{:k}}}
\newcommand{\Xcl}{{X_{:l}}}
\newcommand{\At}{{A^{(t)}}}
\newcommand{\Aini}{{A^{(0)}}}
\newcommand{\Aikini}{{A_{ik}^{(0)}}}
\newcommand{\Aikt}{{A_{ik}^{(t)}}}
\newcommand{\Ajkt}{{A_{jk}^{(t)}}}
\newcommand{\Aiktp}{{A_{ik}^{(t+1)}}}
\newcommand{\Uini}{{U^{(0)}}}
\newcommand{\Ut}{{U^{(t)}}}
\newcommand{\Uikini}{{U_{ik}^{(0)}}}
\newcommand{\Uikt}{{U_{ik}^{(t)}}}
\newcommand{\Ujkt}{{U_{jk}^{(t)}}}
\newcommand{\Uilt}{{U_{il}^{(t)}}}
\newcommand{\Uiktp}{{U_{ik}^{(t+1)}}}
\newcommand{\Ujlt}{{U_{jl}^{(t)}}}
\newcommand{\Vini}{{V^{(0)}}}
\newcommand{\Vt}{{V^{(t)}}}
\newcommand{\Vit}{{V_{i:}^{(t)}}}
\newcommand{\Vikini}{{V_{ik}^{(0)}}}
\newcommand{\Vikt}{{V_{ik}^{(t)}}}
\newcommand{\Vilt}{{V_{il}^{(t)}}}
\newcommand{\Vjkt}{{V_{jk}^{(t)}}}
\newcommand{\Viktp}{{V_{ik}^{(t+1)}}}
\newcommand{\Vjlt}{{V_{jl}^{(t)}}}
\newcommand{\Wt}{{W^{(t)}}}
\newcommand{\Wini}{{W^{(0)}}}
\newcommand{\Wikini}{{W_{ik}^{(0)}}}
\newcommand{\Wikt}{{W_{ik}^{(t)}}}
\newcommand{\Wilt}{{W_{il}^{(t)}}}
\newcommand{\Wiktp}{{W_{ik}^{(t+1)}}}
\newcommand{\Omegaini}{\Omega^{(0)}}

\newcommand{\Ifree}{\mathcal{S}_\mathrm{free}}

\newcommand{\bm}[1]{\boldsymbol{#1}}

\newcommand{\yx}[1]{{\color{blue}(YX: #1)}}


%% macros for vectors
\newcommand{\valpha}{{\boldsymbol{\alpha}}}
\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

%% macros for matrices
\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\vlam}{{\bm{\lambda}}}
\newcommand{\vtheta}{{\bm{\theta}}}
\newcommand{\vell}{{\bm{\ell}}}
\newcommand{\veps}{{\bm{\vareps}}}
\newcommand{\vxi}{{\bm{\xi}}}


%% macros for sets
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}


%
\newcommand{\vareps}{\varepsilon}

%% macros for the real and imaginary parts
\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\rr}{{\mathrm{r}}}

%% macros for math notions and operators
\newcommand{\EE}{\mathbb{E}} % expectation
\newcommand{\RR}{\mathbb{R}} % real
\newcommand{\CC}{\mathbb{C}} % complex
\newcommand{\ZZ}{\mathbb{Z}} % integer
\renewcommand{\SS}{{\mathbb{S}}} % symmetric matrix
\newcommand{\SSp}{\mathbb{S}_{+}} % symmetric positive semi-definite matrix
\newcommand{\SSpp}{\mathbb{S}_{++}} % symmetric positive definite matrix
\newcommand{\sign}{\mathrm{sign}} % sign function
\newcommand{\vzero}{\mathbf{0}} % 0 vector
\newcommand{\vone}{{\mathbf{1}}} % 1 vector

\newcommand{\dist}{\mathrm{dist}}    % distance
\newcommand{\op}{{\mathrm{op}}} % subscript for operator norm
\newcommand{\opt}{{\mathrm{opt}}} % subscript for optimal solution
%\newcommand{\supp}{{\mathrm{supp}}} % support
%\newcommand{\Prob}{{\mathrm{Prob}}} % probability
%\newcommand{\prox}{{\mathbf{prox}}} % proximal map
\newcommand{\Diag}{{\mathrm{Diag}}} % vector -> diagonal matrix
%\newcommand{\diag}{{\mathrm{diag}}} % matrix diagonal -> vector
%\newcommand{\dom}{{\mathrm{dom}}} % domain
%\newcommand{\rank}{\textnormal{rank}}
%\newcommand{\grad}{{\nabla}}    % gradient
\newcommand{\tr}{{\mathrm{tr}}} % trace
\newcommand{\TV}{{\mathrm{TV}}} % total variation
\newcommand{\Proj}{{\mathrm{Proj}}} % projection
\newcommand{\Null}{{\mathrm{Null}}} % null space
\newcommand{\Dim}{{\mathrm{dim}}} % dimension
\newcommand{\etal}{{\textit{et al.}}}
\newcommand{\conj}{{\mathrm{conj}}} % conjugate
\newcommand{\vvec}{{\mathrm{vec}}}
\newcommand{\fold}{{\mathbf{fold}}} % fold into a tensor
\newcommand{\unfold}{{\mathbf{unfold}}} % unfold a tensor
\newcommand{\fit}{{\mathrm{fit}}} % data fitting
\newcommand{\obj}{{\mathrm{obj}}} % data fitting
\newcommand{\round}{{\mathrm{round}}}
% rounding number
\newcommand{\err}{{\mathrm{err}}}
\newcommand{\ST}{\mbox{ subject to }}
\newcommand{\st}{\mbox{ s.t. }}

\newcommand{\ip}[2]{\langle #1 , #2 \rangle}
\newcommand{\vxs}{{\bf x}_{\epsilon,\lambda,q}}
\newcommand{\od}{\frac{d}{dt}}
\newcommand{\pd}{{\partial }}
\newcommand{\rankk}{{\hbox{rank}}}

